Dual-side Sparse Tensor Core

Leveraging sparsity in deep neural network (DNN) models is promising for accelerating model inference. Yet existing GPUs can only leverage the sparsity from weights but not activations, which are dynamic, unpredictable, and hence challenging to exploit. In this work, we propose a novel architecture to efficiently harness the dual-side sparsity (i.e., weight and activation sparsity). We take a systematic approach to understand the (dis)advantages of previous sparsity-related architectures and propose a novel, unexplored paradigm that combines outer-product computation primitive and bitmap-based encoding format. We demonstrate the feasibility of our design with minimal changes to the existing production-scale inner-product-based Tensor Core. We propose a set of novel ISA extensions and co-design the matrix-matrix multiplication and convolution algorithms, which are the two dominant computation patterns in today's DNN models, to exploit our new dual-side sparse Tensor Core. Our evaluation shows that our design can fully unleash the dual-side DNN sparsity and improve the performance by up to one order of magnitude with \hl{small} hardware overhead.

==> 2b_motivation.tex <==
\section{Motivation}

Convolution has played a key role in the training of convolutional neural networks. To best leverage tensor core's matrix-multiply primitives, state-of-the-art DNN acceleration libraries use im2col function to transform convolution into matrix-multiplication (GEMM). We base our dual-side sparse convolution kernel design on an implicit im2col function and outer-product matrix-multiplication.

\begin{figure}[t]
 \centering
  \includegraphics[width=1\linewidth]{draft_img/conv_im2col.pdf}
  \caption{Im2col}
  \label{fig:im2col_conv}
\end{figure}


\subsection{Problems of SpGEMM on GPUs}

implict im2col: Figure~\ref{fig:im2col_conv} (
There are basically two ways to do im2col. Explicit im2col and implicit im2col. \placeholdershort Why we choose implicit im2col. Why we choose outer-product? read SpArch HPCA)\placeholder

Problems of dual-sided sparse: 
Dual-side sparse matrix multiplication requires finding and accessing non-zero elements in matching positions in the two sparse vectors. Previous state-of-the-art \cite{sparten} use . . We address the irregular .
. irregularity and severe imbalance. (tensor core utilization table) \placeholder

\placeholder

\begin{figure}[t]
 \centering
  \includegraphics[width=0.9\linewidth]{draft_img/dp_unit.pdf}
  \caption{Dot product unit in tensor core. Dual-side sparse workloads severely under-utilize tensor core's parallelism.}
  \label{fig:dp_unit}
\end{figure}

\subsection{Problems of im2col}

\begin{figure}[t]
\centering
\subfloat[][Dense im2col]{\includegraphics[scale=0.4]{draft_img/im2col_dense.pdf}\label{fig:im2col_dense}}
\subfloat[][Pseudo code]{
\includegraphics[scale=0.4]{draft_img/im2col_dense_code.pdf}\label{fig:im2col_dense_code}
}
\caption{Im2col on a dense feature map}
\label{fig:im2col_dense_example}
\end{figure}

\begin{figure}[t]
\centering
\subfloat[][CSR im2col]{\includegraphics[scale=0.4]{draft_img/im2col_csr.pdf}\label{fig:im2col_csr}}
\subfloat[][Pseudo code]{
\includegraphics[scale=0.4]{draft_img/im2col_csr_code.pdf}\label{fig:im2col_csr_code}
}
\caption{Im2col on a CSR-encoded feature map}
\label{fig:im2col_csr_example}
\end{figure}



Problems of Im2col: Figure~\ref{fig:im2col_dense_example} and Figure~\ref{fig:im2col_csr_example} and Table~\ref{tab:img2col-sparse-vs-dense} \placeholder

\placeholder



\iffalse
\begin{figure}[t]
\centering
\subfloat[][Inner product]{\includegraphics[width=1\linewidth]{draft_img/baseline_inner.pdf}\label{fig:baseline_inner}}
\newline
\subfloat[][Baseline Implementation (outer-product) ]{
\includegraphics[width=1\linewidth]{draft_img/baseline_outer.pdf}\label{fig:baseline_outer}
}
\caption{Im2col on dense feature map}
\label{fig:im2col_dense_example}
\end{figure}
\fi


==> 6_related.tex <==
\section{Related work}


Some prior efforts exploit dual-sided sparsity on ASIC accelerators but their methods does not fit for architectural features on GPU, especially tensor cores, the specialized hardware for deep learning acceleration. To leverage the matrix-multiplication (GEMM) primitives by tensor core, STOA methods apply im2col function to transform convolution to matrix-multiplication (GEMM). On one hand, many prior work uses Compressed Sparse Row (CSR) format to encode activation feature maps. Since there are a random number of non-zeros in activation feature maps, im2col on CSR-encoded input introduces additional decoding overhead as well as irregular access pattern. Our experiments demonstrate that sparse im2col on CSR-encoded activation on GPU is \note{(to confirm) 10x to 100x} worse than that of its dense counter-parts, which severely degrades the overall performance on sparse convolution. Further more, sparsity pattern in activation dynamically changes with input images, which forbidden offline pre-processing. SCNN . uses dedicated hardware  (CSR encoding format is for im2col and cannot extend to leverage matrix-multiply based tensor core.) \placeholdershort SpArch \placeholdershort. 

On the other hand, dual-side sparse matrix-multiplication (SpGEMM) has severe workload imbalance. \note{(rewrite)} Inner-product does not work. Figure~\ref{fig:outer_product_unit} shows the architectural feature of a basic dot-product unit in tensor core. When both input are sparse, the multiplier and adders are greatly under-utilized. Sparten uses bitmap encoding but its inner-join sequentially conduct multiply and accumulate and thus cannot be applied on tensor core's parallel-multiply-adder-tree architecture. \placeholdershort SparseTrain \placeholdershort 



\begin{table}[t!]
\centering
\caption{Related work}
\label{tab:related_work}
\begin{tabular}{|c|c|c|}
\hline
       & Inner Product & Outer Product \\ \hline
CSR    &  Sparse Tensor Core\cite{sparsetensor}\cite{a100}\cite{mishra2021accelerating}       &  SpArch\cite{sparch} SCNN\cite{scnn} \\ \hline
Bitmap &  Sparten \cite{sparten}  &    \textit{Our approach}   \\ \hline
\end{tabular}
\end{table}


\begin{itemize}

\item[1] SCNN/Sparten, Eyeriss, EIE: dual-side sparse inference. ASIC's method cannot be used in tensor core.

\item[2] SparseTrain, SparCE: dual-side sparse on general-purpose processor (CPU) for training

\item[3] Cambricon-S, Cambricon-X, Scapel, SparseCNN, SSL: single-side sparse inference.

\item[4] Eager-Pruning, PruneTrain: singl-side sparse training.

\item[5] sparse library/software methods on GPUs, cuSparse: single-side sparse for inference

\end{itemize}




==> self_def_command.tex <==
\newcommand{\placeholder}{{\color{gray}{xxx xx xx x xx x xx xxxx xxxx xxx xx xx x xx x xx xxxx xxxxxxx xx xx x xx x xx xxxx xxxx xxx xx xx x xx x xx xxxx xxxx xxx xx xx x xx x xx xxxx xxxx xxx xx xx x xx x xx xxxx xxxx xxx xx xx x xx x xx xxxx xxxx xxx xx xx x xx x xx xxxx xxxx xxx xx xx x xx x xx xxxx xxxx xxx xx xx x xx x xx xxxx xxxx xxx xx xx x xx x xx xxxx xxxx xxx xx xx x xx x xx xxxx xxxx xxx xx xx x xx x xx xxxx xxxx xxx xx xx x xx x xx xxxx xxxx. }}}

\newcommand{\placeholdershort}{{\color{gray}{xxx xx xx x xx x xx xxxx xxxx xxx xx xx x xx x xx xxxx xxxxxxx xx xx x xx x xx xxxx xxxx xxx xx xx x xx x xx xxxx xxxx xxx xxxx xxxx xxx xx xx x xx x xx xxxx xxxx xxx xx xx x xx x xx xxxx xxxx. }}}

\newcommand{\note}[1]{{\color{red}{ #1 }}}


